On Distribution Dependent Sub-Logarithmic Query Time of Learned Indexing

A fundamental problem in data management is to find the elements in an array that match a query. Recently, learned indexes are being extensively used to solve this problem, where they learn a model to predict the location of the items in the array. They are empirically shown to outperform non-learned methods (e.g., B-trees or binary search that answer queries in $O(\log n)$ time) by orders of magnitude. However, success of learned indexes has not been theoretically justified. Only existing attempt shows the same query time of $O(\log n)$, but with a constant factor improvement in space complexity over non-learned methods, under some assumptions on data distribution. In this paper, we significantly strengthen this result, showing that under mild assumptions on data distribution, and the same space complexity as non-learned methods, learned indexes can answer queries in $O(\log\log n)$ expected query time. We also show that allowing for slightly larger but still near-linear space overhead, a learned index can achieve $O(1)$ expected query time. Our results theoretically prove learned indexes are orders of magnitude faster than non-learned methods, theoretically grounding their empirical success.

==> Analysis.tex <==
\section{Analysis}

Assume a set of $n$ points are sampled i.i.d from a distribution $\chi$ defined over a universe $\mathcal{U}$. Let the array, $A$, be the sampled elements sorted in ascending order, with $A[i]$ being $A$'s $i$-th element. Given a query $q\in \mathcal{U}$, the goal is to return $\max_{i\in[n], q \geq A[i]} i$, where $A[0]$ is defined to be $-\infty$. Define $f(q)=\max_{i\in[n], q \geq A[i]} i$


Let the CDF of distribution $\chi$ be $F_{\chi}$ and the empirical CDF be $F_n(x)=\frac{\sum_{i}I_{A[i]\leq x}}{n}$. Note that $f(q)=n\times F_n$ by definition.  

\subsection{Related Work}
In the comparison computational model where an algorithm proceeds by comparison, the problem can be solved in $O(\log n)$ comparisons, while any algorithm solving the problem also requires $\log n$ comparisons in the worst-case. 

Assuming the universe is the finite set $[u]$ of integers, where $u$ denotes the universe size, one can bring down worst-case query time to $O(\log \log u)$ number of operations, which is also proven to be optimal in the cell-probe model.

The assumption that the universe is a finite set of integers exploits the structure of the integer numbers. However, such a structure is not useful for learned approaches and as a result incorrectly quantifies the difficulty of answering queries. For instance, on an array consisting of uniformly spaced data points, one can answer queries with both constant query time and constant space complexity, since a linear function can approximate the query function exactly. The size of the gap is not important, and one can answer queries exactly even for arbitrarily large universes. However, the theoretical framework that relies on the size of the integers for analysis  

The existing theoretical frameworks overlook two aspects. That for a learned approach, the data distribution is the critical source of difficulty in indexing and not the size of the universe.   

\subsection{Distribution Dependent Analysis}
We quantify the difficulty in indexing based on data distribution $\chi$. We break down our analysis into two parts. First, we consider the difficulty of indexing given access to the data distribution. That is, given access to $F_\chi$ (and assuming $F_\chi$ can be evaluated in constant time and space), we ask if one can improve the query time. Second, we consider the difficulty of approximating the distribution itself. 

\subsubsection{Answering Queries Using Data Distribution}
To answer the first question, we present Alg.~X which is able to answer queries in expected query time of $O(\log \log n)$. 


\begin{algorithm}[t]
\begin{algorithmic}[1]
\Require A sorted array $A$ of size $n$ sampled from a distribution $\chi$ with CDF $F_\chi$, a query $q$
\Ensure The predecessor index of $q$ in $A$
\Procedure{Search}{$A$, $q$}
\If{$n\leq 2$}
\State \Return Search the array of 2 elements
\EndIf

\State $p_{min}\leftarrow  F_\chi({A[0]})$
\State $p_{max}\leftarrow  F_\chi({A[-1]})$
\State $F_{\chi}' \leftarrow \frac{F_\chi-p_{min}}{p_{max}-p_{min}}$
\State $i = n\times F_{\chi}'(q)$\label{alg:search:use_dist}
\If{$A[i]=q$}
\State \Return $i$
\EndIf
\If{$A[i]\leq q$}
\State $j = i+\rho\sqrt{n}$
\If{$A[j]\leq q$}\label{alg:search:prob_bound1}
\State \Return BinarySearch($A[j:]$, $q$)
\EndIf
\State \Return Search($A[i:j]$, $q$)
\Else
\If{$A[j] > q$}\label{alg:search:prob_bound2}
\State \Return BinarySearch($A[:j]$, $q$)
\EndIf
\State $j = i-\rho\sqrt{n}$
\State \Return Search($A[j:i]$, $q$)
\EndIf
\EndProcedure
\caption{Search array}\label{alg:search_with_distribution}
\end{algorithmic}
\end{algorithm}

\begin{theorem}
For any query $q\in \mathcal{U}$, on expectation, where the randomness is over the sampling of the array $A$, Alg.~\ref{alg:search_with_distribution} answers queries using $O(\log \log n)$ comparisons and invocations of $F_\chi$. 
\end{theorem}

\textit{Proof}. %For any query $q$, let $T_n$ be the random variable denoting the number of comparisons and invocations of $F_\chi$. Let $B_n$ be the event that the inequality in line \label{alg:search:prob_bound1} or \label{alg:search:prob_bound1} does not hold, and let $p_n=\mathsrc{P}(B_n)$.  Let $B$ be the event that $B_n$, $B_{n^{\frac{1}{2}}}$, ..., $B_{2}$ all hold.  $p(B) = 1-p(\Tilde{B})=1-p(\text{any of $B_{n^{i}}$ doesn't hold})$. By union bound $p(B)\geq 1-de^{-\rho}$ and $p(\Tilde{B})\leq de^{-\rho}$. 
The algorithm recursively proceeds unless it exits to perform a binary search. At the last level of recursion, the size of the array is 2. At every iteration the size of the array is reduced to $\sqrt{n \log\log n}$. For $n\geq 1$, $\log\log n\leq n^{\frac{1}{4}}$, so that the size of the array at the $i$-th recursions is at most $n^{(\frac{3}{4})^i}$, Setting $n^{(\frac{3}{4})^i}\leq2$, we get that $i\leq \frac{\log \log n-\log\log 2}{\log \frac{4}{3}}$. Let $B_i$ denote the event that the algorithm exits to perform binary search at the $i$-th iteration.  Since the size of the array at the $i$-th iteration is $n^{(\frac{3}{4})^i}$, the binary search takes $\log n^{(\frac{3}{4})^i}$. Thus, the expected number of comparisons is $\sum_{i=1}^{\log\log n} 1+ p(B_i,\Tilde{B_{i-1}}, .... \Tilde{B_1})\log n^{(\frac{3}{4})^i}$. Note that 

\begin{align}
p(B_i,\Tilde{B_{i-1}}, .... \Tilde{B_1})=p(B_i|\Tilde{B_{i-1}}, .... \Tilde{B_1})p(\Tilde{B_{i-1}}, .... \Tilde{B_1})\leq p(B_i|\Tilde{B_{i-1}}, .... \Tilde{B_1})
\end{align}

At each iteration of the algorithm, $F_\chi'$ is the CDF from which the items in $A$ are i.i.d sampled. Therefore, by DKW, 

$$
P(|nF_\chi(q)'-nF_n(q)|\geq \rho\sqrt{n})\leq 2e^{-2\rho^2}
$$

$nF_n(q)$ is the actual position of $q$ in $A$ and $nF_\chi(q)$ is the estimated position. DKW implies that with the stated probability the observed position in the array differs at most $\rho\sqrt{n}$ from the estimated position. That is, the event $|nF_\chi(q)-nF_n(q)|\geq \rho\sqrt{n}$ happens if and only if $B_i$ happens, so that their probabilities are the same, i.e.,

$$
p(B_i|\Tilde{B_{i-1}}, .... \Tilde{B_1})\leq 2e^{-2\rho^2}.
$$

Now substitute $\rho=\sqrt{\frac{1}{2}\log\log n}$ so that $e^{-2\rho^2}=\frac{1}{\log n}$, which implies $p(B_i|\Tilde{B_{i-1}})\times \log n^{\frac{1}{2^i}}=1$. 

Now consider the case that we have access to $\hat{f}^{i, j}$ for all $i$ and $j$, that approximates $F_\chi(x)'$ for the sub-array $A[i, j]$ with approximation error $\frac{\sqrt{\log\log (j-i)}}{\sqrt{j-i}}$, so that $|n\hat{f}-nF_{\chi}'|\leq \sqrt{n\log\log (n)}$. 

$$
|n\hat{f}^{i, j}(q)-nF_n(q)| \leq |nF_\chi(q)'-n\hat{f}^{i, j}(q)|+|nF_\chi(q)'-nF_n(q)|
$$

$$
|n\hat{f}^{i, j}(q)-nF_n(q)| \leq \sqrt{n\log\log (n)}+|nF_\chi(q)'-nF_n(q)|
$$

Therefore, $|nF_\chi(q)'-nF_n(q)|\leq \rho\sqrt{n}$ implies
$$
|n\hat{f}^{i, j}(q)-nF_n(q)| \leq 2\sqrt{n\log\log (n)}
$$
So that 

$P(|n\hat{f}^{i, j}(q)-nF_n(q)| \leq 2\sqrt{n\log\log (n)})\geq P(|nF_\chi(q)'-nF_n(q)|\leq \rho\sqrt{n})$

And therefore 

$P(|n\hat{f}^{i, j}(q)-nF_n(q)| \geq 2\sqrt{n\log\log (n)})\leq \frac{1}{\log n}$

Note that the size of the array at the $i$-th level of recursion is at most $16n^{(\frac{3}{4})^i}$, so that binary search takes at most $\log 16n^{(\frac{3}{4})^i}$. 


\qed

\begin{algorithm}[t]
\begin{algorithmic}[1]
\Require A sorted array $A$ of size $n$ sampled from a distribution $\chi$ with CDF $F_\chi$, a query $q$
\Ensure The root node of the learned index
\Procedure{BuildTree}{$A$}
\State $N\leftarrow$ new node with content set to NULL
\If{$n\leq 2$}
    \State $N.content\leftarrow A$
    \State \Return $N$
\EndIf
\State $N.\hat{f}\leftarrow$ piecewise constant function approximating $f_A(q)$ 
\If{Error of $N.\hat{f}>\sqrt{n}$ }
    \State $N.content\leftarrow A$
    \State \Return $N$
\EndIf
\State $N.min\leftarrow A[0]$ 
\State $N.max\leftarrow A[-1]$ 
\State $r\leftarrow 2\sqrt{n}$
\For{$i$ from $0$ to $\frac{n}{r}$}
    \State $n.children[2i]\leftarrow $ BuildTree($A[i\times r:(i+1)\times r]$)
    \State $n.children[2i+1]\leftarrow $ BuildTree($A[i\times r+\frac{r}{2}:(i+1)\times r+\frac{r}{2}]$)
\EndFor
\State \Return $N$
\EndProcedure
\caption{Search array}\label{alg:search_with_distribution}
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
\begin{algorithmic}[1]
\Require The root node, $N$, of a learned index, a query $q$
\Ensure The predecessor index to $q$
\Procedure{Query}{$N$}
\If{$N.content$ is not NULL}
    \State \Return BinarySearch($N.content$)
\EndIf
\State $\hat{i}\leftarrow N.\hat{f}(q)$
\Return Query($\lfloor\frac{2n\hat{i}}{rn}\rfloor$)
\EndProcedure
\caption{Search array}\label{alg:search_with_distribution}
\end{algorithmic}
\end{algorithm}


\subsubsection{Answering Queries Using Model of Distribution}

To answer the second question, we show that a model of data distribution can be used in the place of the data distribution itself. 

We only need to replace line \ref{alg:search_with_distribution} to use a model of the data. Note that there are a total of $O(n^2)$ conditional distributions that need to be modeled (one for every interval). 

\begin{theorem}
    Let $f(x)$ be the p.d.f of $\chi$. Assume $\rho_1 \leq f(x) \leq \rho_2$ for all $x$, where $\rho_1>0$ and $\rho_2<\infty$. Consider a conditional distribution between elements $a_i$ and $a_j$. There exists a piecewise linear function with $k$ pieces, where $k=c\sqrt{j-i}$ whose error is at most $2\frac{\sqrt{\log\log (j-i)}}{\sqrt{j-i}}$
\end{theorem}

\textit{Proof}. Note that, we only need to approximate the range $[a_i, a_j]$. Furthermore, the conditional c.d.f for the range is $\frac{F(x)-F(a_i)}{F(a_j)-F(a_i)}$. We divide the range into $k$ uniformly spaced pieces, so that the $z$-th piece approximates $F$ over $R=[a_i + z\frac{a_j-a_i}{k}, a_i + (z+1)\frac{a_j-a_i}{k}]$, which is an interval of length $\frac{a_j-a_i}{k}$. Let $P_t(x)$ be the constant in the Taylor expansion of $F$ for any $t\in R$. By Taylor's remainder theorem, $|P_t(x)-F(x)|=\frac{F'(c_{x, t})}{F(a_j)-F(a_i)}(x-t)\leq \frac{F'(c_{x, t})}{F(a_j)-F(a_i)}(\frac{a_j-a_i}{k})$ for some $c\in [x, t]$. By mean value theorem, there exist a $c\in [a_i, a_j]$ so that $\frac{F(a_j)-F(a_i)}{a_j-a_i}=F'(c)$. Thus, 

$$|P_t(x)-F(x)|\leq \frac{F'(c_{x, t})}{F(a_j)-F(a_i)}(\frac{x-t}{k})\leq \frac{F'(c_{x, t})}{F'(c)}(\frac{1}{k})\leq \frac{\rho_2}{\rho_1}\frac{1}{k}$$.

Setting $\frac{\rho_2}{\rho_1}\frac{1}{k}\leq \frac{2\sqrt{\log\log(j-i)}}{\sqrt{j-i}}$, we obtain that $k\geq 2\frac{\rho_2}{\rho_1}\sqrt{j-i}$ achieves the desired error.

\qed

\if 0
Since the second derivative is bounded, $|F'(c_{x, t})|\leq |F'(c) +\rho_2 (c-c_{x, t})|$. Therefore, 

$$|P_t(x)-F(x)|\leq \frac{|F'(c) +\rho_2 (c-c_{x, t})|}{|F'c|}(\frac{1}{k})\leq (1+\frac{\rho2}{\rho1})\frac{1}{k}$$

\fi

\if 0

\begin{theorem}
    Let $f(x)$ be the p.d.f of $\chi$. Assume $\frac{d}{dx}\log (f(x))\geq c$ for all $x$. Consider a conditional distribution between elements $a_i$ and $a_j$. There exists a piecewise linear function with $k$ pieces, where $k=\sqrt{c\sqrt{j-i}}$ whose error is at most $2\frac{\sqrt{\log\log (j-i)}}{\sqrt{j-i}}$
\end{theorem}

\textit{Proof.} Note that, we only need to approximate the range $[a_i, a_j]$. Furthermore, the conditional c.d.f for the range is $\frac{F(x)-F(a_i)}{F(a_j)-F(a_i)}$. We divide the range into $k$ uniformly spaced pieces, so that the $z$-th piece approximates $F$ over $R=[a_i + z\frac{a_j-a_i}{k}, a_i + (z+1)\frac{a_j-a_i}{k}]$, which is an interval of length $\frac{a_j-a_i}{k}$. Let $P_t(x)$ be the first-order Taylor expansion of $F$ for any $t\in R$. By Taylor's remainder theorem, $|P_t(x)-F(x)|=F''(c_{x, t})(x-t)^2\leq \frac{F''(c)}{F(a_j)-F(a_i)}(\frac{a_j-a_i}{k})^2$ for some $c\in [x, t]$. Furthermore, by mean value theorem, there exists a $c\in R$ s.t., $\frac{F(a_j)-F(a_i)}{a_j-a_i}=F'(c)$. So,  
$$|P_t(x)-F(x)|\leq \frac{F''(c_{x, t})}{F'(c)}(\frac{a_j-a_i}{k^2})\leq \frac{F''(c_{x, t})}{F'(c)}(\frac{1}{k^2})$$

\fi

\if 0
We model the CDF of the data distribution with piece-wise polynomials

By modelling the cdf of the data distribution as a

That is, if we learn a cdf of a distribution s.t. the cdf can be evaluated in $t_\rho$ and takes space $s_\rho$, while  modeling the true cdf with error at most $\epsilon$, then we can answer indexing queries with runtime $O(x)$. Where $\rho$ is a parameter 

\fi

\begin{theorem}
    There exists a learned index consisting of $O(n^{3.5})$ pieces that answers queries in $O(\log\log n)$ operations on expectation, where the expectation is over the sampling of the array. 
\end{theorem}

\textit{Proof}. There are $n^2$ intervals, for each of which we use the approximation in theorem $X$. Given the approximations, theorem $X$ shows that the number of element accesses and invocation of the function approximators is $\log\log n$. Finally, to account for the number of operations needed to get an estimate from the function approximator, observe that the piece a query falls inside can be found by calculating $\lfloor q-a_i\rfloor$, which is a constant number of operations. Note that the total number of pieces is $\sum_i\sum_j c\sqrt{j-i}$ which is $O(3.5)$. \qed


\begin{theorem}
    Let $f(x)$ be the p.d.f of $\chi$. Assume $\rho_1 \leq f(x) \leq \rho_2$ for all $x$, where $\rho_1>0$ and $\rho_2<\infty$. There exists a learned index consisting of $O(n)$ pieces that answers queries in $O(\log\log n)$ operations on expectation, where the expectation is over the sampling of the array
\end{theorem}

\textit{Proof}. Let the function approximator in line X be the one from theorem X. The size and height of the index are therefore deterministics. XXX

To analyze query time, for any query $q$, consider the path the search algorithm traverses in the tree. 

Let $B_i$ denote the event that the algorithm exits to perform binary search at the $i$-th level.  Since the size of the array at the $i$-th level is $n^{(\frac{3}{4})^i}$, the binary search takes $\log n^{(\frac{3}{4})^i}$. Thus, the expected number of comparisons is $\sum_{i=1}^{\log\log n} 1+ p(B_i,\Tilde{B_{i-1}}, .... \Tilde{B_1})\log n^{(\frac{3}{4})^i}$. Note that 

\begin{align}
p(B_i,\Tilde{B_{i-1}}, .... \Tilde{B_1})=p(B_i|\Tilde{B_{i-1}}, .... \Tilde{B_1})p(\Tilde{B_{i-1}}, .... \Tilde{B_1})\leq p(B_i|\Tilde{B_{i-1}}, .... \Tilde{B_1})
\end{align}

At each iteration of the algorithm, $F_\chi'$ is the CDF from which the items in $A$ are i.i.d sampled. Therefore, by DKW, 

$$
P(|nF_\chi(q)'-nF_n(q)|\geq \rho\sqrt{n})\leq 2e^{-2\rho^2}
$$

$nF_n(q)$ is the actual position of $q$ in $A$ and $nF_\chi(q)$ is the estimated position. DKW implies that with the stated probability the observed position in the array differs at most $\rho\sqrt{n}$ from the estimated position. That is, the event $|nF_\chi(q)-nF_n(q)|\geq \rho\sqrt{n}$ happens if and only if $B_i$ happens, so that their probabilities are the same, i.e.,

$$
p(B_i|\Tilde{B_{i-1}}, .... \Tilde{B_1})\leq 2e^{-2\rho^2}.
$$

Now substitute $\rho=\sqrt{\frac{1}{2}\log\log n}$ so that $e^{-2\rho^2}=\frac{1}{\log n}$, which implies $p(B_i|\Tilde{B_{i-1}})\times \log n^{\frac{1}{2^i}}=1$. 

\qed



\begin{theorem}
    Let $f(x)$ be the p.d.f of $\chi$ with bounded domain [0, 1]. Assume $f(x) \leq \rho$ for all $x$, where $\rho<\infty$. There exists a learned index consisting of $O(n^{1+\epsilon})$ pieces, for any $\epsilon>0$, that answers queries in $O(1)$ operations on expectation, where the expectation is over the sampling of the array. 
\end{theorem}
    
\textit{Proof.} We approximate the query function with a piecewise constant function. We uniformly divide the range [0, 1] into $k$ interval, so that the $i$-th interval is $[i\times \frac{1}{k}, (i+1)\times \frac{1}{k}]$. We set the function value in the $i$-th interval to $f(i\times \frac{1}{k})$. Note that $f(x)$ is a non-decreasing piece-wise constant function, where each step has size 1. Furthermore, steps occur at the points that are sampled. Thus, the error in the $i$-th interval is equal to the number of steps in the interval, which is in turn equal to the number of points sampled in the interval. 

We first bound the probability of the event $E$, that any interval has more than $c$, $c\geq 3$ points sampled in it. The probability, $P_i$ that the $i$-th interval has $c$ points or more is at most

$$
{n \choose c} p_i^c\leq \frac{(en)^c}{c^c}p_i^c
$$

where $p_i=F(\frac{i+1}{k})-F(\frac{i}{k})$ is the probability that a point falls inside the $i$-th interval. Note that by mean value theorem, there exists $c\in [\frac{i}{k}, \frac{i+1}{k}]$ such that $F(\frac{i+1}{k})-F(\frac{i}{k})=f(c)(\frac{1}{k})$. Therefore, $p_i\leq \frac{\rho}{k}$. Thus, by union bound

$$
P(E) \leq \sum_{i=1}^{k}\frac{(en)^c}{c^c}(\frac{\rho}{k})^c=k\frac{(en)^c}{c^c}(\frac{\rho}{k})^c
$$

We would like to get $P(E)\leq \frac{1}{n}$. That is,

$$
k\frac{(en)^c}{c^c}(\frac{\rho}{k})^c\leq \frac{1}{n}
$$

And therefore, 
$$
k\geq n^{\frac{c+1}{c-1}}(\frac{e\rho}{c})^{\frac{c}{c-1}}\geq n^{\frac{c+1}{c-1}}\rho^{\frac{c}{c-1}}
$$

So that 

$$
k\geq n^{1+\frac{2}{c-1}}(\rho)^{1+\frac{1}{c-1}}
$$

Holds for any integer $c\geq 3$. Let $\epsilon=\frac{2}{c-1}$, and therefore,

$$
k\geq n^{1+\epsilon}(\rho)^{1+\frac{\epsilon}{2}}
$$

Thus, for any constant $\epsilon$, $k=O(n^{1+\epsilon})$ number of pieces are sufficient to bound the probability of having more than $c$ points in any interval by $\frac{1}{n}$, which in turn implies that the approximation error for each interval is at most $c$. 

Finally, the query algorithm proceeds as follows. The interval a query falls into is calculated as $k\lfloor\frac{q}{k}\rfloor$. If the interval has more than $c$ points, i.e., if the approximation error is larger than $c$, then we ignore the index and do a binary search. Otherwise, we use the index to find the range of $c$ locations that can contain the query $q$. 

Therefore, the query time of the index is at most $\log c$ with probability $1-\frac{1}{n}$ and $\log n$ with probability $\frac{1}{n}$, so that the expected query time is at most $(\log c)(1-\frac{1}{n})+\log n\times \frac{1}{n}$ which is $O(1)$.

\qed

Note that the algorithm only stores integers, so that the storage cost, except that of storing the array is bounded.


\begin{theorem}
    Let $f(x)$ be the p.d.f of $\chi$ with bounded domain [0, 1]. Assume $f(x) \leq \rho$ for all $x$, where $\rho<\infty$. Assume the data is sampled from a discretized version of $\chi$, where $\bar{F}_\chi(q)=\frac{1}{u}\lfloor\bar{F}_\chi(q)\times u\rfloor$, and assume $u\geq n^{1+\epsilon}$ for some $\epsilon>0$. There exists a learned index consisting of $O(n^{1+\epsilon})$ pieces, for any $\epsilon>0$, that answers queries in $O(1)$ operations on expectation, where the expectation is over the sampling of the array. 
\end{theorem}

\textit{Proof}. We follow a similar strategy as before, but we discretize the beginning and end of each piece. We uniformly divide the range [0, 1] into $k$ interval, so that the $i$-th interval is $(\frac{1}{u}\lfloor\frac{i\times u}{k}\rfloor, \frac{1}{u}\lfloor\frac{(i+1)\times u}{k}\rfloor]$. The maximum length of a range is now $\frac{1}{k}+\frac{1}{u}$, so that $p_i\leq \rho\times (\frac{1}{k}+\frac{1}{u})$. 

Let $k=n^{1+\epsilon'}(\rho)^{1+\frac{\epsilon'}{2}}$, where $0<\epsilon'<\epsilon$ so that for a large enough $n$, $k<u$ and therefore $p_i\leq\frac{2}{k}$. We have for $c\geq 6$ 


$$
P(E)\leq k^{1- c}\frac{(en)^c}{c^c}(2\rho)^{c}\leq k^{1-c}(n)^c(\rho)^{c}
$$

Letting $c=\frac{1+\epsilon'}{\epsilon'}$ and substituting $k$ we get 

$$
P(E)\leq \frac{1}{n}
$$

Finally, note that to find which piece is responsible for a query, we need to perform X which can be done in constant time, and the rest of the algorithm proceeds as before. 
